Multi-group Uncertainty Quantification for Long-form Text Generation

While past works have shown how uncertainty quantification can be applied to large language model (LLM) outputs, the question of whether resulting uncertainty guarantees still hold within sub-groupings of data remains open. In our work, given some long-form text generated by an LLM, we study uncertainty at both the level of individual claims contained within the output (via calibration) and across the entire output itself (via conformal prediction). Using biography generation as a testbed for this study, we derive a set of (demographic) attributes (e.g., whether some text describes a man or woman) for each generation to form such "subgroups" of data. We find that although canonical methods for both types of uncertainty quantification perform well when measuring across the entire dataset, such guarantees break down when examining particular subgroups. Having established this issue, we invoke group-conditional methods for uncertainty quantification -- multicalibration and multivalid conformal prediction -- and find that across a variety of approaches, additional subgroup information consistently improves calibration and conformal prediction within subgroups (while crucially retaining guarantees across the entire dataset). As the problems of calibration, conformal prediction, and their multi-group counterparts have not been extensively explored in the context of long-form text generation, we consider these results to form a benchmark for this setting.

==> tables/list_groups.tex <==
\begin{table}[btp!]
\centering
\caption{List of all groups attributes derived from Wikidata and the values they take on.}
\begin{tabular}{|l|l|}
    \hline
    \textbf{Attribute} & \textbf{Categories} \\ \hline
    \multirow{4}{*}{Nationality} & North America \\
     & Europe/Middle East \\
     & Asia/Pacific \\
     & Latin/South America/Africa \\ \hline
    Number of Wikidata properties & 0-24, 25-49, 50-99, $\geq$100 \\ \hline
    Sex or gender & Male, Female \\ \hline
    Has IMDb ID & True, False \\ \hline
    Plays sport & True, False \\ \hline
\end{tabular}
% \caption{List of all groups attributes derived from Wikidata and the values they take on.}
\label{tab:list_groups}
\end{table}
